Certifying Certainty and Uncertainty in Approximate Membership Query Structures -- Extended Version

Approximate Membership Query structures (AMQs) rely on randomisation for time- and space-efficiency, while introducing a possibility of false positive and false negative answers. Correctness proofs of such structures involve subtle reasoning about bounds on probabilities of getting certain outcomes. Because of these subtleties, a number of unsound arguments in such proofs have been made over the years. In this work, we address the challenge of building rigorous and reusable computer-assisted proofs about probabilistic specifications of AMQs. We describe the framework for systematic decomposition of AMQs and their properties into a series of interfaces and reusable components. We implement our framework as a library in the Coq proof assistant and showcase it by encoding in it a number of non-trivial AMQs, such as Bloom filters, counting filters, quotient filters and blocked constructions, and mechanising the proofs of their probabilistic specifications. We demonstrate how AMQs encoded in our framework guarantee the absence of false negatives by construction. We also show how the proofs about probabilities of false positives for complex AMQs can be obtained by means of verified reduction to the implementations of their simpler counterparts. Finally, we provide a library of domain-specific theorems and tactics that allow a high degree of automation in probabilistic proofs.

==> all.tex <==
\section{Putting It All Together}
\label{sec:all}

As demonstrated in the prior examples, the theorems and tactics we
have constructed in our development happen to form a natural interface
for succinctly reasoning about hash-based probabilistic programs
within Coq.
%
To facilitate the reuse of this tooling, we have packaged the core
components of our code base into a separate library \libname and have
published it on \lname{opam}. The remainder of this section will
discuss this library more detail.

\subsection{The \libname Library}
\label{sec:probh-libr-reas}

Our library is composed of the following modular components, each
focused on handling a different aspect of working with probabilistic
algorithms:

\begin{itemize}
\item \emph{Bounded Length Data Structures.} 
%
  While the \mathcomp library provides a collection of theorems for
  reasoning about fixed length sequences via the $\ccode{Tuple}$ type,
  we found little support for reason about finite sequences with
  varying lengths, \ie, to capture an associative map with a bounded
  capacity.
  %
  As these types of structures often arise when reasoning about
  probabilistic programs, we provide a small library, as a part of
  \libname, to simplify the process of manipulating with
  bounded-length data structures.
  
\item \emph{Probabilistic Computation Framework.} 
  %
  This component consists of our core framework, providing both our
  definition of a deeply embedding probabilistic computation and a
  collection of lemmas encoding the summation patterns.

\item \emph{Hash Vector Library} is a direct application of the
  probabilistic computation framework with a collection of theorems
  about the hash-vector primitive used, in parcticular, in proofs
  about Bloom filters.

\end{itemize}

\noindent
%
Alongside these core components, we also include two specific case
studies to provide concrete examples of how the libary can be used for
practical verification:

%
\begin{itemize}

\item \emph{Bloom filters.} 
  %
  Our first case study is the mechanised proof of the probability of a
  colission in a Bloom filter, as described earlier. We follow the
  proof by Bose \etal\cite{Bose2008Oct}, but axiomatise the fact that
  Stirling numbers of the second kind count the number of surjections
  between sets.
%

%
\item \emph{Counting Bloom filters.} To demonstrate the viability of
  \libname as a standalone library, our second case study uses our
  tooling to prove properties about a standard extension of the Bloom
  filter---Counting Bloom filters.
\end{itemize}

\noindent
%

The sizes each of the library components are given below.

\begin{table}[H]
  \centering
  \begin{tabular}{lcc}
    \toprule 
    Section & \multicolumn{2}{c}{Size (LOC)} \\
     &  Specifications & Proofs  \\
    \midrule
    Notation &  77 & 4 \\
    Hash vectors & 192 & 565 \\
    Bounded containers  & 282 & 1021 \\
    Summation &  485 & 1078 \\
    \midrule
    Bloom filter & 296  & 1803  \\ 
    Counting Bloom filter & 132  & 339 \\
    \bottomrule    
  \end{tabular}
\end{table}


\subsection{Counting Bloom filters in \libname}
\label{sec:probh-libr-reas}

A Counting Bloom filter is an extension of the Bloom Filter to also
support the removal of values~\cite{TarkomaRL12}. It achieves this by
replacing each bit $b_i$ in a Bloom Filter with a counter $d_i$, which
counts the number of times it has been raised.

Insertion proceeds as before, except rather than raising the bits, the
counters are incremented.  Simmilarly, the only change to query is to
treat a counter $d_i$ as raised if its value is greater than 0.  With
this definition, we can implement removal for an element in the set by
simply decrementing all the counters by one.

While the probability of false negatives and positives can also be
analysed for this model, the logical similarities in the insert and
query operations will mean that the proof will mostly follow the same
steps.
%
Instead, for this case study, we opted to demonstrate a more
specialised property---that inserting any value will certainly
increase the sum of all the counters in the filter by a constant
amount:

\begin{theorem}[Certainty of Counter Increments]
\label{thm:counting}

For any counting Bloom filter $\countingbloomfilter$, a value $y$ that
was not previously inserted into $\countingbloomfilter$,
%
if the sum of the values of all counters $d_i$ in
$\countingbloomfilter$ is $l$, then after inserting $y$, the sum of
the counters will certainly increment by $k$.
  %
That is, in terms of probabilities:

{{
\[
  \prob{\sum_{d_i \in \countingbloomfilter} d_i  = l + k } = 1
\]
}}
\end{theorem}

We found that the general proof structure for this case study was
generally the same as for the Bloom filter: (1)~standardise the
computation into normal form, (2)~use the summation patterns to
simplify the computation, (3)~finally, use properties on the
deterministic components of the implementation to complete the proof.
%
The main difference for the second case study was that the
deterministic properties being considered were instead specialised for
Counting Bloom filter. Specifically, in contrast with ordinary Bloom
filters, we had to reason about how the deterministic components of
the implementation would influence the \emph{sum of the counters}
rather than how inserting influences the \emph{raised bits}.
%

These simmilarities between the case studies suggest that our tooling
provided in \libname will be able effectively generalise to larger
classes of probabilistic data structures.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> bitflip.tex <==
\paragraph{Proof of the chance of a bit flip.}

  Consider Theorem ~\ref{thm:sing-bit}, which proves a closed form
  expression of the probability that inserting $l$ elements into an
  empty Bloom Filter will result in a given bit being flipped.

  Fixing a hash vector $\hshs$, an index $\ind$ and a sequence $\xseq$ of
  $l$ distinct values, we will now prove the theorem, that is the probability of
  the bit at $\ind$ being set is given by:
%
  {   \begin{gather*}
        \prob{ ~  \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs)
          \bind  \ccode{bf_get} ~ \ind } = 1 - \left( 1 - \frac{1}{m}\right)^{kl}
      \end{gather*}
}

We can start by simplifying the expression on using one of the
specialised lemmas on conditioned sums (Section~\ref{sec:condsums})
and negating the return value of the computation:

    {   \begin{gather*}
        \prob{ ~  \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs)  \bind \ccode{not} ~  \ccode{bf_get} ~ \ind } = \left( 1 - \frac{1}{m}\right)^{kl}
      \end{gather*}
}

%\vspace{-5pt}
%
\noindent
%
At this point we can perform induction on $l$, where we find again
that the base case is easily dispatched - this time by the fact that
the $i^{\text{th}}$ bit of an empty Bloom filter is by definition
unset.
%
For the inductive case, we can use the positive size bounds to
decompose $\xseq$, and expand the computation:

\begin{align*}
\sum_{\bff',\hshs'} ~\sum_{\bff'',\hshs''} &
\left(
\begin{array}{l}
    \prob{ \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs) = (\bff',\hshs') } ~ \times \\[2pt] 
    \prob{ \ccode{bf_add} ~ x ~  (\bff',\hshs')  = (\bff'',\hshs'') } ~ \times \\[2pt] 
    \prob{ \ccode{not} ~  \ccode{bf_get} ~ \ind ~ \bff'' }
\end{array}
\right)
\\
& = \left( 1 - \frac{1}{m}\right)^{k(l + 1)}
\end{align*}
%\vspace{-5pt}
%
\noindent
%
Distributing the first statement over the inner summation:

{   \begin{align*}
    \sum_{\bff',\hshs'} ~~
    & \left(\prob{ \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs) = (\bff',\hshs') }\right. ~ \times \\ 
    \sum_{\bff'',\hshs''} & \left(\prob{ \ccode{bf_add} ~ x ~  (\bff',\hshs')  = (\bff'',\hshs'') }\right. ~ \times \\
    & \left.\left.\prob{ \ccode{not} ~  \ccode{bf_get} ~ \ind ~ \bff'' } \right)\right)\\
    & \quad \quad = \left( 1 - \frac{1}{m}\right)^{k(l + 1)}
  \end{align*}
}

%
\noindent
%
From here, we can follow Pattern~\ref{lm:plausible} for plausible
outcomes to infer that if the $i^{\text{th}}$ bit of $\bff'$ is set,
then irrespective of the outcome of $\ccode{bf_add}$, the final return
value will be \lname{false}, allowing us to conclude that the
$i^{\text{th}}$ is set, which is a deterministic (\ie,
non-probabilistic) statement and can be expressed as
%
$\ccode{not} ~ \ccode{get_bit_int} ~ i ~ \bff'$.
%
We can the use this fact performing rewriting using
Lemma~\ref{lm:cond-sums} for conditioned sums (in a reverse
direction), thus, introducing an additional probabilistic statement
$\prob{ \ccode{not} ~ \ccode{bf_get} ~ \ind ~ \bff' }$ into our goal
without changing the overall probability:

{ \begin{align*}
    \sum_{\bff',\hshs'} ~~
    & (\prob{ \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs) = (\bff',\hshs') } ~ \times \\ 
    & \prob{  \ccode{not} ~ \ccode{bf_get} ~ \ind ~ \bff' } ~ \times \\ 
    \sum_{\bff'',\hshs''} & (\prob{ \ccode{bf_add} ~ x ~  (\bff',\hshs')  = (\bff'',\hshs'') } ~ \times \\
    & \prob{ \ccode{not} ~  \ccode{bf_get} ~ \ind ~ \bff'' }))\\
    & \quad \quad = \left( 1 - \frac{1}{m}\right)^{k(l + 1)}
  \end{align*}  

\noindent
%
Next we prove an intermediate theorem on the simpler $\ccode{bf_add}$
operation (omitting the proof due to space constraints):

{\small{
\begin{align*}
    \sum_{\bff'',\hshs''}~&
\left(
\begin{array}{l}
\prob{ \ccode{bf_add} ~ x ~  (\bff',\hshs')  = (\bff'',\hshs'') } ~ \times 
\\[2pt]
\prob{ \ccode{not} ~  \ccode{bf_get} ~ \ind ~ \bff'' }                            
\end{array}
\right)
= \left( 1 - \frac{1}{m}\right)^{k}
  \end{align*}
}}

\noindent
%
Applying this rule under the topmost summation, we obtain:

{\begin{align*}
\sum_{\bff',\hshs'} &~~
\left(
\begin{array}{l}
\prob{ \ccode{bf_addm} ~ \xseq ~ (\ccode{bf_new},\hshs) = (\bff',\hshs') } ~ \times \\[2pt] 
\prob{ \ccode{not} ~ \ccode{bf_get} ~ \ind ~ \bff' } ~ \times 
      \left( 1 - \frac{1}{m}\right)^{k}       
\end{array}
\right)
\\
& \quad \quad = \left( 1 - \frac{1}{m}\right)^{k(l + 1)}
\end{align*}  
}

\noindent
%
Then, having removed the dependence on the summand $\bff'$, we can
pull out the non-index-dependent factor and apply the induction
hypothesis to complete the proof.
%
\qed

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> diagram/bloomfilter.tex <==
% feel free to delete if not needed or better way
%  \begin{figure}[H]
    \begin{tikzpicture}
      \coordinate (bloomfilter) at (0,0);
      \coordinate (hashfunctions) at (0,2);
      \coordinate (input) at (0,3);
      \tikzmath{ \bfnodes = 8; \bfhshs =4; \bfboxdim = 0.8; } 

      % draw bloom filter
      \draw ($(bloomfilter) - (\bfboxdim * \bfnodes /2,\bfboxdim /2) $)
            rectangle ++($(\bfboxdim * \bfnodes,\bfboxdim) $);
       \foreach \i in {1,...,\bfnodes}{
         \draw ($(bloomfilter) - (\bfboxdim * \bfnodes /2 - \i * \bfboxdim,\bfboxdim /2) $)
               -- ++($(0, \bfboxdim) $);
                    \pgfmathsetmacro{\subtractresult}{int(\bfnodes-1)}
                    \pgfmathsetmacro{\bfind}{int(\i-1)}
               \node at ($(bloomfilter) - (  \bfboxdim * \bfnodes/2.0 + 0.5 * \bfboxdim  - \i * \bfboxdim,0.0) $) {
                  \tiny\ifthenelse{\i=\bfnodes}{$b_{m-1}$ }{
                    \ifthenelse{\equal{\i}{\subtractresult}}{
                      $\cdots$
                    } {
                      $b_{\bfind}$
                    }
                  }

               };
       }
      %\node at ($(bloomfilter) - (\bfboxdim * \bfhshs,-\bfboxdim ) $) {\textit{Bloomfilter}};

      % draw hashes
      \draw ($(hashfunctions) - (\bfboxdim * \bfhshs /2,\bfboxdim /2) $)
            rectangle ++($(\bfboxdim * \bfhshs,\bfboxdim) $);
       \foreach \i in {1,...,\bfhshs}{
         \draw ($(hashfunctions) - (\bfboxdim * \bfhshs /2 - \i * \bfboxdim,\bfboxdim /2) $)
                -- ++($(0, \bfboxdim) $);
                \pgfmathsetmacro{\subtractresult}{int(\bfhshs-1)}
                \pgfmathsetmacro{\bfind}{int(\i-1)}
                \node at ($(hashfunctions) - (  \bfboxdim * \bfhshs/2 + 0.5 * \bfboxdim  - \i * \bfboxdim,0) $) {
                  \tiny \ifthenelse{\i=\bfhshs}{
                    $f_{k-1}$
                  }{
                    \ifthenelse{\equal{\i}{\subtractresult}}{
                      $\cdots$
                    } {
                      $f_{\bfind}$ 
                    }
                  }
        };                  


       }
       %\node at ($(hashfunctions) - (\bfboxdim * \bfhshs,-\bfboxdim ) $) {\textit{Hashes}};



       \node (x) at ($(input) + (0, \bfboxdim/2)$) {$x$};

       \draw (x) -- ($(input)$);
       %draw input arrows
       \foreach \i in {1,...,\bfhshs}{
         \draw[->] ($(input)$) -|
         ($(hashfunctions) - (  \bfboxdim * \bfhshs/2 + 0.5 * \bfboxdim  - \i * \bfboxdim,-\bfboxdim/2) $);
       }
       

       % draw random output arrows
       \draw
       ($(hashfunctions) - (\bfboxdim * \bfhshs /2 + 0.5 * \bfboxdim - 1 * \bfboxdim,\bfboxdim /2) $) edge
       [out=270,in=90,->] 
       ($(bloomfilter) - (  \bfboxdim * \bfnodes/2 + 0.5 * \bfboxdim  - 8 * \bfboxdim,-\bfboxdim/2) $) ;

       \draw
       ($(hashfunctions) - (\bfboxdim * \bfhshs /2 + 0.5 * \bfboxdim - 2 * \bfboxdim,\bfboxdim /2) $) edge
       [out=270,in=90,->] 
        ($(bloomfilter) - (  \bfboxdim * \bfnodes/2 + 0.5 * \bfboxdim  - 2 * \bfboxdim,-\bfboxdim/2) $);

       \draw
       ($(hashfunctions) - (\bfboxdim * \bfhshs /2 + 0.5 * \bfboxdim - \bfhshs * \bfboxdim,\bfboxdim /2) $) edge
       [out=270,in=90,->] 
        ($(bloomfilter) - (  \bfboxdim * \bfnodes/2 + 0.5 * \bfboxdim  - 5 * \bfboxdim,-\bfboxdim/2) $);


       
       
    \end{tikzpicture}
%  \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> diagram/framework.tex <==
% feel free to delete if not needed or better way
\begin{figure}[H]
  \centering
    \begin{tikzpicture}[
      module/.style={shape=rectangle,draw=black,semithick, align=center}
      ]
       \node[module] (AMQ) at (0,0) {AMQ};
       \node[module] (HashVec) at (0,-1) {Hash Vector};
       \node[module] (Hash) at (-3,-1) {Hash};
       \node[module] (MultiHash) at (3,-1) {Multiplexed Hash};
       \node[module] (QF) at (-3,-2.5) {QF};
       \node[module] (BF) at (-1.5,-2.5) {BF};
       \node[module] (CBF) at (1.5,-3.5) {CBF};
       \node[module] (BlockedAMQ) at (3,-2.5) {BlockedAMQ};

       \draw[->] (Hash) --  +(0,0.5) -| (AMQ);
       \draw[->] (HashVec) --  +(0,0.5) -| (AMQ);
       \draw[->] (MultiHash) --  +(0,0.5) -| (AMQ);
       \draw[->] (QF) -- (Hash);
       \draw[->] (BF) -- +(0,0.5) -| (HashVec);
       \draw[->] (CBF) --  +(0,1.5) -| (HashVec);
       \draw[->] (BlockedAMQ) -- (MultiHash);
       \draw[<-,dashed,color=red,thick] (BF) -- +(1.5,0.0) node[color=black,fill=white,below=0.25] {reduction} |- (CBF);
       \draw[->,dashed,color=green,thick] (BlockedAMQ)
       --  +(2.0,0.0)
       |-
       node[color=black,fill=white,above=0.0] {composition}
       (AMQ);
    \end{tikzpicture}
  \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> hshconsistency.tex <==
\paragraph{Proof of hash consistency.}

Consider Theorem~\ref{thm:reducing-hash-vector} that stated that
re-hashing a seen value certainly produces a consistent result.
%  
Fixing a hash vector $\hshs$, a value $x$, and a vector of outputs
$\inds$ such that $\hshs$ maps $x$ to $\inds$, we will now prove this
theorem, that we can be certain that hashing $x$ via $\hshs$ will
produce $\inds$. Formulated in terms of probabilities:

  { %\small  
      \[
        \prob{\ccode{hash_vec_int} ~ x ~\hshs = (\hshs, \inds)} = 1
      \]
}

\noindent
%
The proof proceeds by induction on the length $k$ of the hash-vector.
The base case is trivially dispatched, leaving just the inductive
step.
  %
Then using the length bounds to determine that $\hshs$ and $\inds$ are
non-empty (as $(k + 1) > 0$), we can decompose each one into a
corresponding head and tail. This allows distributing the fact that
$\hshs$ maps $x$ to $\inds$ over the heads and tails.
%
Our goal then becomes proving that if $\hsh$ maps a value $x$ to an
output $\ind$ and $\hshs$ maps $x$ to the vector $\inds$, then the we
can be certain that hashing $x$ via $\hsh :: \hshs$ will produce
$\ind :: \inds$:
%
{%\small   
    \begin{gather*}
%
        \prob{\ccode{hash_vec_int} ~ x ~ (\hsh ::\hshs) = (\hsh ::\hshs,\ind ::\inds) } = 1
%
\end{gather*} }  

\vspace{-5pt}
%
\noindent
%
As \ccode{hash_vec_int} applies the hashing operation over each pair
of value $x$ and hash vector element $\hsh$ in the input, we can
normalise the computation into its sub-steps:
%
{   \begin{align*}
            \sum_{\hsh',\ind'}
            & \prob{\ccode{hash}  ~ x ~\hsh = (\hsh',\ind')} \times
               \prob{\ccode{ret} ~ (\hsh',\ind') = (\hsh,\ind)}~ \times \\
            & \prob{\ccode{hash_vec_int} ~  x ~\hshs = (\hshs,\inds) } = 1
  \end{align*}
}

\vspace{-5pt}
%
\noindent
%
Following the sequential composition Pattern~\ref{lm:seqcomp}, we can
eliminate this intermediate return operation, thus the goal
%
{
  \begin{gather*}
    \prob{\ccode{hash} ~ x ~\hsh = (\hsh,\ind)} \times \quad \\
 \quad   \prob{\ccode{hash_vec_int} ~  x ~\hshs = (\hshs,\inds) } = 1
  \end{gather*}
}

\vspace{-5pt}
%
\noindent
%
From the definition of the \ccode{hash} and the fact that $\hsh$ maps
$x$ to~$\ind$, the first factor can be further reduced to~$1$,
leaving:
%
{
\begin{align*} \prob{\ccode{hash_vec_int} ~ x ~
     \hshs = (\hshs,\inds) } = 1
  \end{align*}
}

\vspace{-5pt}
%
\noindent
%
The proof can then be completed by a straightforward application of
the inductive hypothesis.
\qed



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> hshuniform.tex <==
\begin{paragraph}{Proof of hash uniformity}
  Consider Theorem \ref{thm:uniform-hash-vector} which guarantees the
  hash outputs a uniform distribution if the input value has not been
  hashed before:
{\small   \begin{gather*}
    \forall (hshs, hshs': \fintuple{k}{\ccode{HashState} ~ n}),\\
    (inds: \fintuple{k}{\ordnat{m}}), x, \\
    \ccode{hash_unseen} ~ x ~ hshs,\\
    hshs' = hshs \leftarrow (x,inds),\\
    \prob{\ccode{hash_vec_int} ~ x ~ hshs = (hshs',inds)} = \left(\frac{1}{m}\right)^{k}
  \end{gather*}
}
  Performing induction on $k$, we can again eliminate the base case by
  the fact that all empty sequences are equal.
  % 
  This leaves just the inductive case, where we can use the length
  bounds to decompose the lists and simplify the expression:
{\small   \begin{gather*}
    \ccode{find} ~ x ~ hsh = \ccode{Some} ~ ind  \wedge \ccode{hash_unseen} ~ x ~ hshs,\\
    hsh'  = (\ccode{put} ~ x ~ ind ~ hsh)  \wedge  hshs' = (hshs \leftarrow (x,inds)),\\
      \prob{  \ccode{hash_vec_int} ~ x ~ (hsh :: hshs) = (hsh' :: hshs', ind :: inds) } \\
        = \left(\frac{1}{m}\right)^{k + 1}
  \end{gather*}
}
  Then using the \textbf{sequential composition} pattern, we can
  distribute and simplify the probabilistic computation into a
  product:
{\small   \begin{gather*}
    % \begin{align*}
      \prob{ \ccode{hash} ~ x ~ hsh = (hsh', ind) } ~ \times 
             \prob {\ccode{hash_vec_int} ~ x ~ hshs = (hshs', inds)}
    % \end{align*} 
    \\
    = \left(\frac{1}{m}\right)^{k + 1}
  \end{gather*}
}
   Expanding the definition of $\ccode{hash}$, we find that it evaluates to a uniform distribution over $\ordnat{m}$:
{\small   \begin{gather*}
     \left(\frac{1}{m}\right) \times 
     \prob {\ccode{hash_vec_int} ~ x ~ hshs = (hshs', inds)} \\
    = \left(\frac{1}{m}\right)^{k + 1}
  \end{gather*}
}
  At this point, the conclusion trivially follows by application of
  the inductive hypothesis.

\end{paragraph}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> paper.log.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> todo.tex <==

\section*{TODOs}
\label{sec:todos}

Here are some ideas on how the paper needs to be reworked to emphasise
the new story with the general framework for AMQ verification (do we
want to rebrand it from \libname to something else?). Below, I outline
the flow of the paper along with sections sizes (we only have 20 pages).

\begin{enumerate}
\item The intro [2-2.5pp] is almost okay. It needs to be made more
  ambitious to emphasise a large class of AMQs that we're tackling.
  Towards its end we will write about the framework, enumerating all
  data structures it accommodates. We will also claim the following as
  contributions:

  \begin{itemize}
  \item The systematic decomposition of AMQs and their properties,
    emphasising the proofs obtained ``for free'' and reductions.
  \item A number of case studies, none of which have been previously
    verified
  \item A number of novel data structures composed out of verified
    ones, along with their proofs.
  \item Proof automation for big sums
  \item Proof of Stirling numbers form
  \end{itemize}

\item The Overview [2pp] is good -- almost no changes required.

\item Sections 3 and 4 [4pp] need to be significantly shortened and
  merged together under the title \textbf{Encoding of AMQs and Their
    Properties}. The story still can go about Bloom filter (avoiding
  the general module structure as much as mossible), with a number of
  forward pointers about how it's going to be generalised. Only a
  couple of most interesting theorems about hash-vectors should stay,
  the rest can go into the appendix. Also, we should probably not
  trumpet hash-vectors that much as a big contrib, but rather state
  that it's a convenient design choice.

\item Section entitled \textbf{FRAMEWORKNAME at Large} [3pp]. Here
  should come a section about the design of the framework, showing the
  diagram and explaining all the interfaces, first referring to Bloom
  filter. It is a good place to show some meta-theorems and discuss
  the requirements for getting \emph{No-False-Negatives for Free}
  (there should be a paragraph on that). It would be also nice to pick
  another data structure (e.g., Counting filter) and quickly go
  through its components showing how modules need to be instantiated.

\item Section \textbf{Proof Patterns and Automation} [3pp]. Here we should
  spend a couple of pages talking about bigsums, lemmas, patterns and
  the tactics that support them. A very short proof of something that
  uses exclusively the tactics would be nice.

\item \textbf{Case Studies} [2.5pp] -- Show Blocked filters and their
  composition. Discuss how the properties compose. Present statistics
  on the proofs sizes (perhaps, broken into components according to
  the framework), and proof checking time. It's also a good time to
  tell some anecdotes about the most useful libraries and tricks
  you've discovered and how that reduced the proof sizes.

\item \textbf{Discussion and Related Work}[1.5pp]. Here, we first want to
  tell a sad story about all those broken proofs, enumerating all of
  them with references. 
  %
  The we add our related work (with some cuts).

\item \textbf{Conclusion}[0.3pp] Super-short, no need for future work.

  
\end{enumerate}



==> toolbox.tex <==

\section{Examples of Probabilistic Proofs}
\label{sec:proof}

% Therefore, for transitioning back to the Big Picture, once you’re done with Section 5,
% you may want remind the reader why do we care at all by showing a shortened derivation
% (no more that 4-6 rewritings) of one of the important statements (Theorem 4.3, perhaps)
% using the described summation patterns and their rewritings.
% While doing so, you should refer consistently to the subsections of Section 5,
% that outline the corresponding principles.
% The goal of this exercise is to convey that the facts we have captured and
% encapsulated as a library in Coq directly map to the human intuition when proving facts like Thm 4.3. 
Having described core theorems of our development, this section
presents examples of how they can be combined to efficiently prove
properties on probabilistic programs.



% \kg{I've presented the proof for theorem 4.3 below, but I don't think
%   it is the best example (only really uses one rule):}

\subsection{Derivation of Library Primitives}

To illustrate how our patterns of probabilistic reasoning interact in
practice, let us first consider how they are used to derive one of the
core theorems on hash vectors.

\input{hshconsistency}

% \input{hshuniform}

\subsection{General Proofs of Hash-Based Algorithms}

The modularity of our proof strategy means that even the more involved
theorems can be proven cleanly by decomposing the goals into smaller
intuitive steps.

% \kg{Having written it out, it might not be the best example}

\input{bitflip}


\paragraph{Proof of probability of false positives.}
%
The proof of Theorem~\ref{lemma:enc-fpos} about false positives
utilises our patterns in a simmilar way, employing
Pattern~\ref{lm:sum-bind} for bind decomposition to rewrite the
computation into the normal form.
%
The proof differs slightly in that it also uses
Lemmas~\ref{lm:sum-cons} and~\ref{lm:sum-concat} for
{distributing sums over cons} and {distributing sums over
  concatenation} to reduce the property over the probabilistic
computation into a simpler form, before utilising the axiomatized
properties of Stirling numbers second kind to complete the proof.
  %
  As the proof is significantly more involved, the full details have
  been ommited from this manuscript but are available in our
  accompanying development.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

